A Statistical Framework for District Energy Long-term Electric Load Forecasting

An accurate forecast of electric demand is essential for the optimal design of a generation system. For district installations, the projected lifespan may extend one or two decades. The reliance on a single-year forecast, combined with a fixed load growth rate, is the current industry standard, but does not support a multi-decade investment. Existing work on long-term forecasting focuses on annual growth rate and/or uses time resolution that is coarser than hourly. To address the gap, we propose multiple statistical forecast models, verified over as long as an 11-year horizon. Combining demand data, weather data, and occupancy trends results in a hybrid statistical model, i.e., generalized additive model (GAM) with a seasonal autoregressive integrated moving average (SARIMA) of the GAM residuals, a multiple linear regression (MLR) model, and a GAM with ARIMA errors model. We evaluate accuracy based on: (i) annual growth rates of monthly peak loads; (ii) annual growth rates of overall energy consumption; (iii) preservation of daily, weekly, and month-to-month trends that occur within each year, known as the 'seasonality' of the data; and, (iv) realistic representation of demand for a full range of weather and occupancy conditions. For example, the models yield an 11-year forecast from a one-year training data set with a normalized root mean square error of 9.091%, a six-year forecast from a one-year training data set with a normalized root mean square error of 8.949%, and a one-year forecast from a 1.2-year training data set with a normalized root mean square error of 6.765%.

==> packages_and_newcommands.tex <==
%% Packages and Newcommands

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%packages
\usepackage{color}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{verbatim}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{theorem}
\usepackage{tabu}
\usepackage{tabularx}
\usepackage{accents}
\usepackage{array}
\usepackage{float}
\usepackage{subfig}
\usepackage{lineno}
\usepackage{hhline}
\usepackage{caption}
\usepackage{subcaption}
\DeclareRobustCommand{\ubar}[1]{\underaccent{\bar}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%newcommands

\newcommand{\f}{\textit{f}\hspace{0.01in}}
\newcommand{\cI}{{\cal{I}}}
\newcommand{\cJ}{{\cal{J}}}
\newcommand{\cT}{{\cal{T}}}
\newcommand{\cP}{{\cal{P}}}
\newcommand{\cS}{{\cal{S}}}
\newcommand{\cW}{{\cal{W}}}
\newcommand{\cM}{{\cal{M}}}
\newcommand{\cF}{{\cal{F}}}
\newcommand{\cV}{{\cal{V}}}
\newcommand{\tco}{\textcolor{orange}}
\newcommand{\tcb}{\textcolor{blue}}
\newcommand{\tcr}{\textcolor{red}}
\newcommand{\tcg}{\textcolor{green}}
\newcommand{\tck}{\textcolor{black}}
\newcommand{\tcp}{\textcolor{purple}}
\newcommand{\minlpmod}{{$(\cW)$}}
\newcommand{\submod}{{$(\cS)$}}
\newcommand{\mastermod}{{$(\cM)$}}


\newcommand{\assignmirror}{{X}}
\newcommand{\cleaningperiod}{{E}}
\newcommand{\buyvehicle}{{P}}
\newcommand{\ftcrew}{{F}}
\newcommand{\seascrew}{{W}}
\newcommand{\usecollection}{{U}}
\newcommand{\useveh}{{M}}

\newcommand{\vehicle}{{v}}
\newcommand{\vehicles}{{\cV}}
\newcommand{\numvehicles}{{V}}

\newcommand{\mirror}{{\f}}
\newcommand{\mirrors}{{\cF}}
\newcommand{\nummirrors}{{F}}

\newcommand{\tperiod}{{t}}
\newcommand{\tperiods}{{\cT}}
\newcommand{\numtperiods}{{T}}

\newcommand{\vehset}{{i}}
\newcommand{\vehsets}{{\cI}}
\newcommand{\numvehsets}{{I}}

\newcommand{\vtype}{{j}}
\newcommand{\vtypes}{{\cJ}}
\newcommand{\numvtypes}{{J}}


\newcommand{\soilfunc}{{g}}
\newcommand{\rate}{{\bar{s}_{\mirror\tperiod}}}
\newcommand{\subobj}{c^{\text{\submod}}}
